InterMask: 3D Human Interaction Generation via Collaborative Masked Modeling

Generating realistic 3D human-human interactions from textual descriptions remains a challenging task. Existing approaches, typically based on diffusion models, often produce results lacking realism and fidelity. In this work, we introduce InterMask, a novel framework for generating human interactions using collaborative masked modeling in discrete space. InterMask first employs a VQ-VAE to transform each motion sequence into a 2D discrete motion token map. Unlike traditional 1D VQ token maps, it better preserves fine-grained spatio-temporal details and promotes spatial awareness within each token. Building on this representation, InterMask utilizes a generative masked modeling framework to collaboratively model the tokens of two interacting individuals. This is achieved by employing a transformer architecture specifically designed to capture complex spatio-temporal inter-dependencies. During training, it randomly masks the motion tokens of both individuals and learns to predict them. For inference, starting from fully masked sequences, it progressively fills in the tokens for both individuals. With its enhanced motion representation, dedicated architecture, and effective learning strategy, InterMask achieves state-of-the-art results, producing high-fidelity and diverse human interactions. It outperforms previous methods, achieving an FID of $5.154$ (vs $5.535$ of in2IN) on the InterHuman dataset and $0.399$ (vs $5.207$ of InterGen) on the InterX dataset. Additionally, InterMask seamlessly supports reaction generation without the need for model redesign or fine-tuning.

==> sec/intro.tex <==
\section{Introduction}

\label{sec:intro}

% In this chapter, we present InterMask, a novel collaborative masked generation framework designed to synthesize 3D physical human interactions conditioned on natural language descriptions. We begin by reaffirming the motivation for modeling 3D human interactions and explaining the rationale for employing a masked generative framework. Subsequently, we delve into the modeling of interaction generation using our novel approach. This includes a comprehensive explanation of the architectural components of our method, the training algorithm for each component, and the inference algorithm used to generate human interactions based on natural language descriptions.
%3D physical human interactions involve complex exchange of synchronized actions between multiple individuals in a shared space. These interactions are characterized by intricate spatial and temporal dependencies, where the actions of one person simultaneously influence and respond to the actions of another. Examples of such interactions include shaking hands, dancing, or engaging in a physical sport like boxing. These interactions are crucial for various applications in animation, virtual reality, robotics, and human-computer interaction, where realistic and believable human movements enhance user experience and interaction fidelity. Despite its importance, the field of 3D human interaction modeling is still in its infancy, primarily due to limited availability of large-scale, high-quality motion capture datasets. Most available human interaction datasets~\citep{Marcard_2018_ECCV_3dpw, guo2022expi, 9156717_chi3d, liu2019ntu, 9093627_duetdance, ghosh2023remos} have various limitations including insufficient quantity, inadequate motion capture quality, limited action categories and lack of textual annotations. Recently, the introduction of InterHuman~\citep{liang2024intergen} and InterX~\citep{xu2024inter} datasets has been a significant breakthrough. These datasets provide accurate motion capture samples and accompanying natural language descriptions for a wide range of interaction scenarios. These scenarios range from daily life interactions like shaking hands and passing objects to more professional contexts such as dancing, boxing, and fencing. These datasets open doors for further exploration of joint modeling of natural language and human interactions due to their sufficient scale and diversity.
% While human interaction generation is only recently gaining attention, the field of single-person motion generation has seen significant progress. There has been extensive research in recent years on creating realistic and diverse human motion sequences. Various generative modeling frameworks, including Variational Autoencoders (VAEs)~\citep{guo2022generating, petrovich2022temos}, Generative Adversarial Networks (GANs)~\citep{Shiobara2021HumanMG}, Autoregressive Transformers~\citep{jiang2023motiongpt, zhang2023t2m, guo2022tm2t}, and Diffusion models~\citep{tevet2022human,chen2023executing,zhang2022motiondiffuse}, have been explored for this task. Recently, MoMask~\citep{guo2024momask} introduced a masked generative framework for human motion generation. This significantly improved motion quality and inference efficiency over diffusion or autoregressive models by predicting multiple tokens simultaneously, thus reducing the number of inference steps required.

Digital human interaction generation is a fundamental task in computer vision and computer graphics, with applications in animation, virtual reality, robotics, and sports. Although recent advances in human motion generation~\citep{tevet2022human,guo2024momask,guo2022generating,pinyoanuntapong2024mmm,zhang2023t2m,petrovich2022temos} have enabled the production of diverse, high-quality single-person motions from textual descriptions, when coming to two-person, it remains a significant challenge. During two-person interactions, the motion of one individual depends not only on their own state but also on the state of their partner. Furthermore, precise spatial positioning becomes crucial, particularly when close contact is involved. The complexity and nuances of human interactions introduce a higher degree of spatial and temporal interdependence comparing to single-person motion.
%, indicating the need for approaches specifically designed for interaction modeling.

%3D physical human interactions involve a synchronized exchange of actions between individuals, characterized by intricate spatial and temporal dependencies. %In human-human interactions, the current movement of one only not depend on the status of itself, but also the status of its partner. 
%, where each person's actions simultaneously influence the respond to the other. 
%Examples include shaking hands, dancing, or engaging in sports like boxing. Creation of these interactions are essential in fields such as animation, virtual reality, robotics, and human-computer interaction, where realistic, high-fidelity movements enhance user experience. %Despite the progress in single-person motion generation in recent years
%Despite the challenges in modeling human interactions due to limited large-scale datasets, recent contributions like InterHuman~\citep{liang2024intergen} and InterX~\citep{xu2024inter} have provided improved motion capture and natural language annotations, allowing for a broader range of scenarios compared to earlier datasets~\citep{Marcard_2018_ECCV_3dpw, guo2022expi, 9156717_chi3d, liu2019ntu, 9093627_duetdance, ghosh2023remos}. Concurrently, single-person motion generation has seen significant advances, with models such as Variational Autoencoders (VAEs)~\citep{guo2022generating, petrovich2022temos}, Generative Adversarial Networks (GANs)~\citep{Shiobara2021HumanMG}, Autoregressive Transformers~\citep{jiang2023motiongpt, zhang2023t2m, guo2022tm2t}, and Diffusion models~\citep{tevet2022human,chen2023executing,zhang2022motiondiffuse} driving improvements in motion realism. Recently, MoMask~\citep{guo2024momask} and MMM~\citep{pinyoanuntapong2024mmm} introduced a framework that enhances both efficiency and quality by reducing inference steps through parallel token prediction.

%While it might seem straightforward to extend single-person motion generation techniques to multi-person interactions, the complexity, and nuance in human interactions introduce a higher degree of spatial and temporal influence. In multi-person interactions, the current pose of one not only depends on the status of itself, but also the status of its partner. Moreover, the precision of the spatial locality of the poses is much more critical because relative distance and orientation play a significant role in human interactions. Additionally, the interaction space is exponentially larger than that of single-person motion, involving a broader range of possible actions and reactions. Previous works, such as ComMDM~\citep{shafir2023human}, have demonstrated that methods designed for single-person motion generation do not scale well to interactions between multiple individuals. The higher-order complexity of human interactions necessitates new approaches tailored specifically for interaction modeling. 


Existing works on human-human interaction generation commonly employ diffusion models. ComMDM~\citep{shafir2023human}, using a limited amount of interaction data, learns a small neural layer that bridges two pretrained single-person motion diffusion models. On the contrary, InterGen~\citep{liang2024intergen}  is specifically tailored for two-person motion generation, which uses cooperative diffusion transformers to model individual motions conditioned on the latent features of their partner's movements. Recently, in2IN~\citep{ruiz2024in2in} conditioned the interaction diffusion model not only on the overall interaction description but also on LLM-generated descriptions for each individual. Additionally, it leveraged motion priors learned from single-person motion datasets like HumanML3D~\citep{guo2022generating}. In MoMat-MoGen~\cite{cai2024digital}, motions were retrieved based on textual inputs from supplementary motion datasets and subsequently refined for realism and interaction quality. A few other works~\citep{shan2024towards, fan2024freemotion} have extended these methods to generate motions for any number of subjects from textual prompts. Despite these substantial efforts, the generated two-person interactions still fall short of achieving satisfactory realism and fidelity.

%InterGen~\citep{liang2024intergen}, alongwith introducing the InterHuman dataset, established a baseline for text-to-interaction generation with its diffusion-based approach. It utilizes cooperative diffusion transformers to model individual motions conditioned on the hidden representations of motion of the interacting partner. Building upon this work, two concurrent works, in2IN~\citep{ruiz2024in2in} and MoMat-MoGen~\citep{cai2024digital}, have proposed enhancements to InterGen's performance. The former leverages additional data in the form of single-person motion descriptions generated by a Large Language Model (LLM)~\citep{minaee2024large}, complementing the interaction descriptions provided in the InterHuman dataset. This approach enables more robust control over generated motions and facilitates pretraining of a single-person motion prior, using text-to-motion datasets like HumanML3D~\citep{guo2022generating}. On the other hand, MoMat-MoGen employs a combination of motion matching and generation techniques, prioritizing fidelity over diversity. Similar to in2IN, it utilizes individual annotations to retrieve motion sequences from a prior database learned from supplementary datasets, subsequently refining these motions to enhance interaction coherence while maintaining a degree of diversity. Though with these substantial prior efforts on human interaction generation, the generated two-person interactions are yet to be satisfied.
%While both in2IN and MoMat-MoGen present innovative solutions that incorporate LLM reasoning capabilities and leverage additional single-person motion annotations, it is important to note that they diverge from the original objective of simultaneously generating motions for both interacting individuals based solely on a holistic textual description.

%In this work, we introduce a new scheme of two-person motion generation, InterMask, a novel framework for generating 3D human interactions from natural language descriptions more effectively and efficiently. InterMask proposes a masked modeling approach, built upon two foundational components, to generate 3D human interactions. The first component is a custom 2D motion Vector Quantized Variational AutoEncoder (\emph{2D motion VQ-VAE}). The VQ-VAE creates a single-person motion codebook that maps continuous 3D motion sequences onto discrete motion tokens, resulting in a compact, discrete representation space for high-dimensional motion data. Unlike previous motion VQVAEs~\citep{guo2024momask, zhang2023t2m, jiang2023motiongpt, zhang2023motiongpt, pinyoanuntapong2024mmm}, our 2D motion VQ-VAE retains the spatial dimension of motion sequences. It does this by representing each timestep as a collection of vectors, with one vector for each joint, instead of a single vector for all joints. This approach improves the precision in modeling spatial relations within interactions. The second component is the Interactive Spatio-Temporal Transformer (\emph{ISTFormer}), which is a collaborative masked generative transformer. ISTFormer models interactions between two people by learning the text-conditional probability distribution of the discrete tokens obtained from the 2D motion VQ-VAE. It uses a masked token prediction surrogate objective in a collaborative setting and introduces novel Spatio-Temporal attention layers. These layers enable more accurate modeling of the 2-dimensional tokens for each person.

% In human interactions, the accuracy of joint positions is far more critical than in single-person motion, as interactions are primarily defined by the spatial relationships between various body parts of the interacting individuals. For instance, during a handshake, the participants must face each other and be positioned close enough for their hands to meet when extended.


In this work, we present \emph{InterMask}, a novel framework based on generative masked modeling in discrete space. InterMask consists of two stages. First, we learn a shared VQ-VAE to transform each individual's motion sequence into a 2D discrete token map (\Cref{sec:vqvae}). In previous motion VQ-VAE approaches~\citep{guo2022tm2t,zhang2023t2m,jiang2023motiongpt,zhang2023motiongpt,guo2024momask,pinyoanuntapong2024mmm}, each motion is represented as a matrix of shape $N\times D$, where $N$ is the number of poses and 
$D$ is the dimensionality of the pose feature vector. 1D convolutions are then applied to these matrices, resulting in 1D motion token sequences, where each token encodes only temporal context for all joints over a short range. In contrast, we represent a motion as a matrix of shape $N\times J \times d$, where $J$ is the number of joints and $d$ is the dimensionality of joint features. By using 2D convolutions, we preserve both the temporal and spatial dimensions in the VQ-VAE, producing a 2D token map. This approach allows tokens in the 2D map to capture the context of specific body parts in short temporal ranges, promoting better joint locality. This is particularly important in interactions, as the motions are more sensitive to relative body part positions (e.g., hands) between two individuals. Additionally, high-fidelity movement details can be better retained in local motion tokens, as empirically evidenced in~\Cref{tab:ablation_vq}. The second stage of InterMask involves a Transformer with specifically designed architecture for modeling interaction, and a dedicated masking scheme to generate motion tokens of two persons.%, detailed in~\Cref{sec:transformer}.

% \chuan{In what follows, first describe the generative masking scheme, and lastly your design of model, then inference process.}

\chuan{I feel the next two paragraphs can be merged. Make the presentation more succinct. Avoid redundant presentation.} We first flatten the 2D token maps of both individuals and concatenate them with a separator token in-between. We utilize a two-round masking regime to mask the concatenated tokens of both individuals. In the first round, we apply either \emph{random masking}, guided by a scheduling function, or \emph{interaction masking}, where only the tokens from one individual are masked while the other remains unmasked, promoting the learning of inter-person dependencies. In the second masking round, a portion of the predicted tokens from the first round is retained, and the rest are masked again for subsequent prediction, namely \emph{step unroll masking}. This iterative process aligns the training with the progressively prediction and re-masking of the inference phase. After masking, the tokens of both individuals are turned into embeddings and then collaboratively processed using the proposed Inter-M Transformer, consisting of $\mathbf{L}$ blocks. Each block starts with a self-attention module~\citep{vaswani2017attention}, capturing long-range dependencies within and between each individual's tokens. The token embeddings of both individuals are then split and processed through shared spatio-temporal and cross-attention modules. The spatio-temporal attention models spatial and temporal relationships within each individual, while the cross-attention captures dependencies between the two. This design ensures effective learning of both intra- and inter-person interactions along both spatial and temporal dimensions, as empirically evidenced in~\Cref{tab:ablation_trans}. Finally, a probability distribution over $|\mathcal{C}|$ codebook entries is obtained for each token using softmax. 
\begin{figure*}[t]
	\begin{center}
	\includegraphics[width=\linewidth]{img/teaser_small.pdf}
     % % \vspace{-1.0em}
        \end{center}
	\caption{Teaser. \chuan{Much better. I feel the figure can be denser. Otherwise it occupied too much space. Meanwhile, for the layout, would it be better if we put two half-width figures at the bottom, instead of the middle? I am not sure, but you may have a look. In addition, the three-line captions could adjusted to two-line if we lengthen the text box. The time line indicator took a bit too much vertical space. One rule of thumb is to keep the overall layout regular in shape, avoiding too much empty space or irregular shape.}}
	\label{fig:teaser}
	 % % \vspace{-1.5em}
\end{figure*}

During inference, we use a progressive generation mechanism over a fixed number of $I$ iterations, beginning with all tokens of both individuals fully masked. At each iteration, all tokens are predicted simultaneously, and the most confident predictions are retained, while the remaining tokens are masked again. The masking ratio is controlled by a scheduling function that gradually reduces the number of masked tokens at each step, continuing until all tokens have been predicted. Once the motion tokens for both individuals are generated, their corresponding codes are retrieved from the learned codebook $\mathcal{C}$. These codes are then passed through the VQ-VAE decoder to reconstruct the final motion sequences for both individuals.


\chuan{Remember when we talk about InterMask, the most important things is the generative masking, which makes the framework intrinsically different from others. Always put generative masking at the first.} The main contributions of this work can be summarized as follows. First, we present the InterMask framework, which proposes a novel 2D motion token map and the Inter-M Transformer, along with a two-stage masking regime. This framework allows for effective modeling of spatial and temporal dependencies in both intra- and inter-person dynamics. Second, InterMask achieves state-of-the-art results in generating high-fidelity and realistic text-conditioned human interactions, demonstrating its capability to model complex interactions with high precision. Empirically it achieves an FID of 5.15 (vs 5.54 in~\citet{ruiz2024in2in}) on InterHuman and FID of 0.399 (vs 5.207 in~\cite{liang2024intergen}) on InterX. Third, the framework offers flexibility by supporting related tasks such as reaction generation, without requiring any task-specific finetuning or modifications to the architecture.

%InterMask offers significant advantages over diffusion or autoregressive models. Unlike autoregressive transformers, which use unidirectional attention to past tokens and predict only the next token in a single forward pass, ISTFormer utilizes a bidirectional attention mechanism. This allows ISTFormer to attend to both past and future tokens and predict all masked tokens simultaneously, enhancing both the model's expressivity and efficiency. By employing simultaneous token prediction, InterMask significantly reduces the number of inference steps compared to autoregressive and diffusion models, making it more suitable for real-time applications. Furthermore, since InterMask uses single-person motion tokens, it works out-of-the-box for human reaction generation without the need for any task-specific fine-tuning.

% Our main contributions can be summarized as follows: TODO
% \begin{itemize}
%     \item \textbf{InterMask Framework:} A novel masked generative modeling approach for generating 3D human interactions from natural language descriptions.
    
%     \item \textbf{2D Motion VQ-VAE:} A custom 2-dimensional VQVAE that retains the spatial dimension of motion sequences, allowing for precise modeling of spatial relations in interactions.
    
%     \item \textbf{ISTFormer:} A collaborative masked generative transformer with novel Spatio-Temporal attention layers, improving the modeling of interactions and enabling efficient, simultaneous prediction of masked tokens.

%     \item \textbf{Efficiency and Expressivity:} Enhances model expressivity and efficiency over autoregressive and diffusion models, making it suitable for real-time applications by reducing inference steps.

%     \item  \textbf{Versatile Task Support:} InterMask inherently supports related tasks, including reaction generation based on a single person’s motion and temporal inpainting, without requiring task-specific fine-tuning or modifications to the framework, demonstrating its flexibility and robustness in diverse scenarios.
%\end{itemize}


